Supervised and Unsupervised protocols for hetero-associative neural networks

This paper introduces a learning framework for Three-Directional Associative Memory (TAM) models, extending the classical Hebbian paradigm to both supervised and unsupervised protocols within an hetero-associative setting. These neural networks consist of three interconnected layers of binary neurons interacting via generalized Hebbian synaptic couplings that allow learning, storage and retrieval of structured triplets of patterns. By relying upon glassy statistical mechanical techniques (mainly replica theory and Guerra interpolation), we analyze the emergent computational properties of these networks, at work with random (Rademacher) datasets and at the replica-symmetric level of description: we obtain a set of self-consistency equations for the order parameters that quantify the critical dataset sizes (i.e. their thresholds for learning) and describe the retrieval performance of these networks, highlighting the differences between supervised and unsupervised protocols. Numerical simulations validate our theoretical findings and demonstrate the robustness of the captured picture about TAMs also at work with structured datasets. In particular, this study provides insights into the cooperative interplay of layers, beyond that of the neurons within the layers, with potential implications for optimal design of artificial neural network architectures.

==> sections/coop-vecchia.tex <==
{\color{red} bozza di sezione, da riscrivere e da rendere meno ripetitiva}

In this section, we analyze the emergent behavior of our multipartite network in the context of the TAM model, using three different methodologies: the one-step magnetization approximation, Monte Carlo simulations, and analytical solving of the self-consistency equations.

The one-step magnetization approximation represents a first description of the system, whose behavior appears to be essentially ``\emph{selfish}". In this formulation, the magnetization of each level depends mainly on the local entropy, with minimal influence exerted by the other levels. This perspective suggests a dynamic in which individual layers act independently of each other, without significant interaction with each other.

Monte Carlo simulations, on the other hand, offer a more nuanced view, showing partial interaction between the layers. Although each layer retains some autonomy, coupling effects between layers are observed, suggesting the presence of an initial sign of cooperative behavior. However, this methodology fails to fully capture the interdependencies between layers and their collective effect on the overall dynamics of the network.

Finally, analytical resolution of the phase diagrams, based on the self-consistency equations, reveals complete cooperative behavior. In this description, the resilience of each layer is not simply determined by local entropy, but emerges as the result of a complex interaction among all layers in the network. In particular, it is observed that levels with high entropy can benefit from the presence of levels with lower entropy, thus improving their overall performance.

This progression, from local approximations to full analytical description, clearly shows how the emergence of cooperation is an intrinsic property of the system, which becomes evident only through rigorous global analysis. The following sections will delve into each of these approaches, highlighting their limitations and their ability to describe network dynamics.

\subsection{One-step magnetization}
The one-step magnetization approach provides an initial approximation of the network's retrieval behavior by considering the dominant influence of local entropy. In this framework, each layer's magnetization is primarily governed by its own entropy parameter, with minimal contributions from other layers. This results in a \emph{self-centered} dynamic, where the network exhibits an apparent lack of cooperation among different levels.

\textcolor{red}{DA SNELLIRE, richiamare formule esistenti e dire che stiamo considerando il caso simmetrico con interazioni unitarie}
To illustrate this effect, we analyze the one-step magnetizations obtained in the supervised setting (see Sec. \ref{subsec:montecarlo}).
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{ImagesLearning/CountorPlotMagn.png}
    \caption{Contour plot of magnetization values as a function of entropy values, $\rho_1,\rho_2,\rho_3 \in [0,1]$, in the supervised setting. We also set $\gamma=0.25$. For simplicity we have set $\rho_2=\rho_3$ and
    consequently, the magnetization
    values corresponding to layer $\bm{\tau}$ are identical to those of the layer $\bm{\phi}$ (left). We observe that the increase in entropy $\rho_{2/3}$ marginally influences the decrease in the value of $m_{\xi^1}^{\sigma}$ whereas the decrease is more substantial as entropy $\rho_1$ increases (right). An analogous situation but referring to magnetizations $m_{\eta^1}^{\tau}$ and $m_{\chi^1}^{\phi}$: here we observe that the dominant entropy is $\rho_{2/3}$.}
    \label{Magnerho}
\end{figure}
\noindent
In this context, the magnetization equations for the supervised scenario are given by
\begin{equation}
\label{magnsingtonoisee}
\begin{array}{lll}
   m_{\xi^1}^\sigma &= \mathrm{erf}\left[\dfrac{1}{\sqrt{2}}\dfrac{1}{\sqrt{\rho_1  +\gamma\dfrac{( \a^2 +\b^2)}{\mu_{1,\sigma}^2}}}\right], \\
  m_{\eta^1}^\tau &= \mathrm{erf}\left[\dfrac{1}{\sqrt{2}}\dfrac{1}{\sqrt{\rho_2  +\gamma\theta^2\dfrac{( \a^2 +\c^2)}{\mu^2_{1,\tau}}}}\right], \\
  m_{\chi^1}^\phi &= \mathrm{erf}\left[\dfrac{1}{\sqrt{2}}\dfrac{1}{\sqrt{\rho_3  +\gamma\alpha^2\dfrac{( \b^2 +\c^2)}{\mu^2_{1,\phi}}}}\right],
  \end{array}
\end{equation}
whereas for the unsupervised counterpart, they take the form
\begin{align}
m^\sigma_{\xi^1}(\rho_1, \rho_2, \rho_3,\gamma) = \text{erf}\left[\frac{1}{\sqrt{2}\sqrt{\rho_1 + \gamma\frac{(1 + \rho_2)(1 + \rho_3)}{(\sqrt{1 + \rho_2} + \sqrt{1 + \rho_3})^2}\left(\frac{1 + \rho_{12}}{1 + \rho_2} + \frac{1 + \rho_{13}}{1 + \rho_3}\right)}}\right], \\
m^\tau_{\eta^1}(\rho_1, \rho_2, \rho_3,\gamma) = \text{erf}\left[\frac{1}{\sqrt{2}\sqrt{\rho_2 + \gamma\frac{(1 + \rho_1)(1 + \rho_3)}{(\sqrt{1 + \rho_1} + \sqrt{1 + \rho_3})^2}\left(\frac{1 + \rho_{12}}{1 + \rho_1} + \frac{1 + \rho_{23}}{1 + \rho_3}\right)}}\right], \\ 
m^\phi_{\chi^1}(\rho_1, \rho_2, \rho_3,\gamma) = \text{erf}\left[\frac{1}{\sqrt{2}\sqrt{\rho_3 + \gamma\frac{(1 + \rho_1)(1 + \rho_2)}{(\sqrt{1 + \rho_1} + \sqrt{1 + \rho_2})^2}\left(\frac{1 + \rho_{13}}{1 + \rho_1} + \frac{1 + \rho_{23}}{1 + \rho_2}\right)}}\right].
\end{align}

These equations highlight that the retrieval performance of each layer is predominantly controlled by its own entropy parameter. As shown in Fig. \ref{Magnerho}, the magnetization values of each layer are only weakly influenced by the entropy levels of the other layers, reinforcing the self-centered nature of this approximation.





\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{ImagesLearning/Cooperativity .pdf}
    \caption{Monte Carlo simulations showing magnetization behavior as a function of load, \(\gamma\), for different entropy values \(\rho_1\), \(\rho_2\), and \(\rho_3\), in the supervised setting. The symmetric network structure is characterized by \(N_1 = N_2 = N_3 = 1000\), with identical parameters \(M_1 = M_2 = M_3 = 20\) and \(\beta = 1000\). Each plot corresponds to one of the three network layers: \(\bm\sigma\) (left), \(\bm\tau\) (center), and \(\bm\phi\) (right). In the plots, the blue curves represent the low-entropy regime (\(\rho = 0.0\)), the orange curves depict an intermediate-entropy configuration (\(\rho_1 = 0.0, \rho_2 = \rho_3 = 0.2\)), and the red curves correspond to the high-entropy regime (\(\rho = 0.2\) across all layers). The results highlight the differences in retrieval performance across layers under varying entropy distributions. Notably, the intermediate regime demonstrates a partially cooperative effect: while layer \(\bm\sigma\) retains a higher magnetization compared to \(\bm\tau\) and \(\bm\phi\), its performance surpasses that in the fully noisy scenario. These findings emphasize the interconnectedness of the layers, where the noise levels in one layer influence retrieval in others. Such dynamics underline the cooperative behavior intrinsic to the network, which is only partially captured by Monte Carlo simulations, hinting at deeper underlying principles better addressed by self-consistency equations.}
    \label{montecarlolayersiaiutano}
\end{figure}

\subsection{Monte Carlo simulations}
 In Fig. \ref{montecarlolayersiaiutano} we present a Monte Carlo's simulation of the situation, in the supervised scheme,  offering an intermediate view between self-consistent results and those obtained under the one-step approximation. In the figure we observe that the network’s retrieval performance in the regime $(\rho_1,\rho_2,\rho_3)=(0.0,0.2,0.2)$, depicted by the orange line, lies
between the performance in low-entropy (blue line) and high-entropy
(red line) regimes, indicating communication among the three layers. However, we also note that the retrieval capabilities of layer $\bm{\sigma}$ in the
intermediate scenario are superior
to those of the other two layers. This ``\emph{partially cooperative}"
behavior is again a consequence of the approximations inherent in the
Monte Carlo method. While Monte Carlo simulations fall short in
capturing the nuances of this problem, we believe that self-consistency
equations within the realm of statistical mechanics provide a powerful
tool to unravel the emergent behaviors exhibited by these networks.


\subsection{Phase diagrams results} \label{subsec:coopPhaseDiag}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{ImagesLearning/diag_fase_sup_variRho_3layer.png}
    \caption{Numerical solution of equations \eqref{seldefinitive} and \eqref{seldefinitive1}. The phase diagrams illustrate the retrieval regions for each layer, represented by \(\bm\sigma\), \(\bm\tau\), and \(\bm\phi\), under different configurations of the noise parameters \(\rho_1\), \(\rho_2\), and \(\rho_3\). The first row corresponds to \(\rho_1 = \rho_2 = \rho_3 = 0\), representing the absence of noise. The second row sets \(\rho_1 = 0\) and introduces noise in the second and third layers with \(\rho_2 = \rho_3 = 0.20\). In the third row, noise is uniformly distributed across all layers with \(\rho_1 = \rho_2 = \rho_3 = 0.20\). The diagrams clearly show how increasing noise in one or more layers influences the retrieval performance in the others, demonstrating the cooperative behavior of the network. Specifically, the interplay between \(\beta^{-1}\) and \(\gamma\) highlights the system's robustness and adaptation. For all cases, the network parameters are set to \(\alpha = \theta = 1\) and \((g_\sigma, g_\tau, g_\phi) = (1, 1, 1)\), emphasizing the intrinsic symmetry of the interactions between the layers.}
    \label{DifferentRho}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth+0cm]{ImagesLearningUnsup/self/diag_fase_unsup_variRho_3layer.png}
    \caption{Numerical solutions of the self-consistency equations \eqref{eq:selfMagnSigma}-\eqref{eq:selfQPhi} in the $(\gamma,\beta)$ plane for each row, with fixed parameters $(\alpha,\theta) = (1,1)$. The phase diagrams illustrate the retrieval regions for each layer, represented by \(\sigma\), \(\tau\), and \(\phi\), under different configurations of the noise parameters \(\rho_1\), \(\rho_2\), and \(\rho_3\).
	In the top row, we set low entropies for each of the three layers, specifically $(\rho_1,\rho_2,\rho_3) = (0.2, 0.2, 0.2)$. In the middle row, we use $(\rho_1, \rho_2, \rho_3) = (0.2, 0.6, 0.6)$, while in the bottom row, we select $(\rho_1, \rho_2, \rho_3) = (0.6, 0.6, 0.6)$, corresponding to high entropy across all layers. The diagrams clearly show how varying noise in one or more layers influences the retrieval performance in the others, demonstrating the cooperative behavior of the network.}
    \label{fig:TAMLayerHelpEO}
\end{figure}


In this section, we explore a newly identified emergent property within the class of \( k \)-partite networks, focusing on its manifestation in the TAM model.

A detailed examination of the phase diagrams, parameterized by the entropy values across the distinct layers \( \bm\sigma \), \( \bm\tau \), and \( \bm\phi \) (see Figs. \ref{DifferentRho}, \ref{fig:TAMLayerHelpEO}), reveals an intriguing phenomenon. Specifically, the network's retrieval capabilities exhibit a transition between low-entropy and high-entropy regimes. Importantly, the retrieval performance of each layer does not merely reflect the entropy of its corresponding dataset but is instead governed by the collective interplay of entropy distributions across all layers. 

Notably, when the network is in a heterogeneous entropy configuration, we observe a redistribution effect: the retrieval performance of the layer associated with the most structured dataset decreases, while the layers with higher entropy benefit from this interaction. This results in a more balanced retrieval performance across the network. This emergent effect highlights the intrinsic cooperative nature of the system, wherein the presence of a more structured layer can enhance the performance of noisier layers, fostering a form of mutual reinforcement. Conversely, when entropy is uniformly distributed at high levels across all layers, the retrieval performance is uniformly suppressed, underscoring the limitations imposed by excessive noise. 

We propose the term ``\emph{cooperativeness}" to describe this emergent property of the network, a feature that inherently arises from the mutual influence of the layers' entropy levels. This cooperative behavior is not merely a byproduct of parameter tuning but an intrinsic characteristic of the multipartite network structure, which only becomes evident through a comprehensive analytical treatment of the system’s self-consistency equations.






==> sections/coop.tex <==



